Neuromorphic High-Frequency 3D Dancing Pose Estimation in Dynamic Environment

As a beloved sport worldwide, dancing is getting integrated into traditional and virtual reality-based gaming platforms nowadays. It opens up new opportunities in the technology-mediated dancing space. These platforms primarily rely on passive and continuous human pose estimation as an input capture mechanism. Existing solutions are mainly based on RGB or RGB-Depth cameras for dance games. The former suffers in low-lighting conditions due to the motion blur and low sensitivity, while the latter is too power-hungry, has a low frame rate, and has limited working distance. With ultra-low latency, energy efficiency, and wide dynamic range characteristics, the event camera is a promising solution to overcome these shortcomings. We propose YeLan, an event camera-based 3-dimensional high-frequency human pose estimation(HPE) system that survives low-lighting conditions and dynamic backgrounds. We collected the world's first event camera dance dataset and developed a fully customizable motion-to-event physics-aware simulator. YeLan outperforms the baseline models in these challenging conditions and demonstrated robustness against different types of clothing, background motion, viewing angle, occlusion, and lighting fluctuations.

==> contents/application.tex <==

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.6\linewidth]{images/outdoor_res.png}
    \caption{Outdoor result samples. The first two rows are data recorded in day time, while the last two are during the night.}
    \label{fig:outdoor_res}
\end{figure}

% Besides MiDHP and NiDHP, we collect a smaller dataset in outdoor environments with a DVS camera to show the applicability outside. Part of the data was recorded in the daytime, while the rest was collected at night. We guarantee that each major movement comes with some background noise such as like one or multiple cars passing in the distance. 
Besides the real-world indoor test set, we also tested \emph{YeLan} qualitatively on our collected outdoor dataset. This dataset is recorded at a roadside where many cars pass by, and we can use these cars as background activities while the foreground participant is moving. There are cars of different types riding at different speeds, and our participant is in his casual wearings instead of the uniformed black close-fitting T-shirt and shorts used in the indoor dataset. In this section, to increase the generalizability, the model we use is the one pretrained on the synthetic dataset and fine-tuned on the real-world indoor dataset. As Fig. \ref{fig:outdoor_res} shows, the mask prediction network works well in both day and night settings and successfully rejects events generated by cars and other background noises. In this way, our 3D human pose estimation network could also make predictions stably without being disturbed by the background activities. Moreover, although the build-in RGB camera suffered a lot from the motion-blurring problem in low-lighting conditions, \emph{YeLan}'s performance is not affected much thanks to the event camera's scotopic characteristic and representation TORE's history preservation ability.


% Therefore, we cannot directly show the overlay figures with event representation and predicted skeleton when presenting the results. Instead, we plot the predicted skeleton in 3D coordinates separately, please only focus on the relative position of joints. 
% Also, be aware that the 3D figure may have perspective, and the resulting image could be slightly different from the imagination. 
% Results are shown in Fig. \ref{fig:outdoor_res}, where we can still see that the model works well in terms of joints' relative position.

% This dataset have neither corresponding ground truth labels, nor camera extrinsic matrix, as we do not have motion capture devices and an original point for reference. 

==> contents/bio.tex <==
% @ Fran

% Human eye is more efficient in capturing moving objs
% Human can easily focus on foreground objects but filter out the other contents
% Human can still see in dark/very bright env
% Human eye is somehow similar to DVS

In primate biological systems, there are significant and sophisticated systems dedicated to interpreting and responding to visual input. Light enters the eye and is first processed on the retina using a combination of photoreceptive cell types. The two dominant photoreceptors are rods, which enable vision in low-light conditions, and cones, which are active in high-light conditions and translate small, medium, and long-wavelength light into color \cite{lamb2016rods}. Rods have a higher spatial density on the outer edges of the retina, while cones are concentrated in the center of the retina. The combination of these two photoreceptors signals light changes in the visual field. It transmits these signals, via the optic nerve, to the occipital lobe to be processed in the visual cortex \cite{kandel2000principles}. The primary visual cortex is located in the posterior cerebrum. By having visual processing begin at the back of the brain, basic light signals are translated from changes in light wavelength and photon densities into complex visual representations as processing moves towards anterior neural processing areas along dorsal and ventral processing streams \cite{kandel2000principles}. Throughout this visual processing architecture, light is broken down and processed to track objects as they move across the retina efficiently; shift focus between foreground and background objects, and maintain quality vision in both high and low light conditions. In this paper, our novel design seeks to mimic the ability of rod photoreceptors to respond to single-photon changes by efficiently processing DVS camera single-pixel changes to process and predict body position in both high and low light conditions. 

% [1]
% @article{lamb2016rods,
%   title={Why rods and cones?},
%   author={Lamb, Trevor D},
%   journal={Eye},
%   volume={30},
%   number={2},
%   pages={179--185},
%   year={2016},
%   publisher={Nature Publishing Group}
% }

% [2]
% Kandel, E. R., Schwartz, J. H., Jessell, T. M., Siegelbaum, S., Hudspeth, A. J., & Mack, S. (6th.). (2021). Principles of Neural Science (Ch. 22, pp. 521-544). New York: McGraw-Hill.

% [3]
% Kandel, E. R., Schwartz, J. H., Jessell, T. M., Siegelbaum, S., Hudspeth, A. J., & Mack, S. (6th.). (2021). Principles of Neural Science (Ch. 24, pp. 564-580). New York: McGraw-Hill.

% (to be edited) 

% @book{kandel2000principles,
%   title={Principles of Neural Science},
%   author={Kandel, Eric R and Schwartz, James H and Jessell, Thomas M and Siegelbaum, Steven and Hudspeth, A James and Mack, Sarah and others},
%   volume={4},
%   year={2000},
%   publisher={McGraw-hill New York}
% }


